Bayesian MISE convergence rates of Polya urn based density estimators: asymptotic comparisons and choice of prior parameters

Mixture models are well-known for their versatility, and the Bayesian paradigm is a suitable platform for mixture analysis, particularly when the number of components is unknown. Bhattacharya (2008) introduced a mixture model based on the Dirichlet process, where an upper bound on the unknown number of components is to be specified. Here we consider a Bayesian asymptotic framework for objectively specifying the upper bound, which we assume to depend on the sample size. In particular, we define a Bayesian analogue of the mean integrated squared error (Bayesian MISE), and select that form of the upper bound, and also that form of the precision parameter of the underlying Dirichlet process, for which Bayesian MISE of a specific density estimator, which is a suitable modification of the Polya-urn based prior predictive model, converges at a desired rate. As a byproduct of our approach, we investigate asymptotic choice of the precision parameter of the traditional Dirichlet process mixture model; the density estimator we consider here is a modification of the prior predictive distribution of Escobar & West (1995) associated with the Polya urn model. Various asymptotic issues related to the two aforementioned mixtures, including comparative performances, are also investigated.

==> comparison.tex <==




\section{Comparison between MISE's of EW and SB}
\label{sec:comparison_sb_ew}

As claimed in \ctn{Sabya10a} and \ctn{Sabya10}, the SB model is much more
efficient than the EW model in terms of computational complexity and ability to 
approximate the true underlying clustering or regression.
%Though the form of the model we have used for this paper is different from MB and MRB, 
%here also we are interested to see 
%whether SB model is more efficient than EW model in terms of less $MISE$. Recall that the forms of $MISE$ are
Here we investigate the conditions under which the model of SB beats that of EW in terms of $MISE$.
In particular, we provide conditions which guarantee that each term of the order of $MISE(EW)$
dominates the corresponding term of the order of $MISE(SB)$ (for any two sequences $\{a^{(1)}_n\}$ 
and $\{a^{(2)}_n\}$
we say that $a^{(1)}_n$ dominates $a^{(2)}_n$ if $a^{(2)}_n/a^{(1)}_n\rightarrow 0$ as $n\rightarrow\infty$).

For the purpose of comparison we will use the same values of $b_n$, $\sigma_n$, $\epsilon_n$, for all $n$, for both SB and EW model,
in a way such that both the $MISE$'s converge to 0.

%Note that we have chosen $\epsilon_n$ in EW model such that $\frac{\epsilon_n}{1-\epsilon_n} < 
%O\left(\left[e^{\frac{n(a+c_1)^2}{2{b_n}^2}}\frac{(\alpha+n)^n}{(\alpha)^n H_0^n}\right]^{-1}\right)$. 

\begin{comment}
\begin{equation}
O(MISE(EW))=\left(\frac{\alpha}{\alpha+n}\right)^2+B_n+\epsilon_n^*+\sigma_n^2  \nonumber
\end{equation}

\begin{equation}
O(MISE(SB))=MB_M+\left(1-\frac{1}{M}\right)^n\left(\frac{\alpha+M}{M}\right)^M+\epsilon_M^*+\sigma_n^2 \nonumber
\end{equation}
To compare the $MISE$'s is not an easy task due to the forms. However we can simplify this comparison by performing term by term comparison
of the $MISE$'s. 
\end{comment}

\begin{lemma}
\label{lemma:compare1}
Let $\alpha=n^{\omega}$, $M=n^b$, where $\omega <1$, $b<1$, and $\omega <b$. Then,\\
$\frac{\epsilon_M^*}{\epsilon_n^*}\rightarrow 0$.
\end{lemma}
\begin{proof}
The proof follows from simple applications of L'Hospital's rule.
\end{proof}

\begin{comment}
\begin{eqnarray}
&\frac{\epsilon_M^*}{\epsilon_n^*}&=\dfrac{\left(\frac{\alpha+M}{\alpha}\right)^M\frac{1}{B_0^M}}{\left(\frac{\alpha+n}{\alpha}\right)^n\frac{1}{B_0^n}}
=B_0^{n-M} \left(\frac{\alpha}{\alpha+n}\right)^n \left(\frac{\alpha+M}{\alpha}\right)^M  \label{eq:epsilon}
\end{eqnarray}

Denote $r(n)=\dfrac{\left(\frac{\alpha+M}{M}\right)^M \frac{1}{B_0^M}}{\left(\frac{\alpha+n}{\alpha}\right)^n \frac{1}{B_0^n}}=
B_0^{n-M} \frac{\left(\frac{\alpha}{\alpha+n}\right)^n}{\left(\frac{\alpha}{\alpha+M}\right)^M}$.
Taking logarithm, 
\begin{eqnarray}
&&\log(r(n))=n \log\left(\frac{\alpha}{\alpha+n}\right)-M\log\left(\frac{\alpha}{\alpha+M}\right)\nonumber\\
&\Rightarrow& \log(r(n))=n \log\left(\frac{\alpha}{\alpha+n}\right) \left[1-\frac{n^b \log(1+n^{b-\omega})}{n\log(1+n^{1-\omega})}\right]
\label{eq:lp1}
\end{eqnarray}


Now,
\begin{eqnarray}
\frac{n^b \log(1+n^{b-\omega})}{n\log(1+n^{1-\omega})}=\frac{\log(1+n^{b-\omega})}{n^{1-b}\log(1+n^{1-\omega})}
\label{eq:lp2}
\end{eqnarray}
Note that if $\omega<1$, $b<1$, $b> \omega$, then R.H.S of equation (\ref{eq:lp2}) goes to 0, as $n\rightarrow 0$. Thus \\
$\left[1-\frac{n^b \log(1+n^{b-\omega})}{n\log(1+n^{1-\omega})}\right]\rightarrow 1$. \\

Again $n\times \log\left(\frac{\alpha}{\alpha+n}\right)\rightarrow -\infty$ (can be shown by simple application of L'Hospital's rule).
So, we have\\
$n\times \log\left(\frac{\alpha}{\alpha+n}\right) \left[1-\frac{n^b \log(1+n^{b-\omega})}{n\log(1+n^{1-\omega})}\right]\rightarrow -\infty$.
Thus $r(n)\rightarrow 0$. Since $B_0<1$, $B_0^{n-M}\rightarrow 0$ and hence $\frac{\epsilon_M^*}{\epsilon_n^*}\rightarrow 0$.

\end{comment}

\begin{lemma}
\label{lemma:compare2}
%Suppose $M(=n^b)>\alpha(=n^\omega)$, such that $M(\alpha+M)\cong M^2$ and $\alpha+n\cong n$. Then
%$B_n>MB_M$ if $M<n^{1/2}$.
Let $M=n^b$ and $\alpha=n^{\omega}$, where $b>\omega$. Then $B_n>MB_M$ if $M<\sqrt{n}$. 
\end{lemma}
\begin{proof}
The proof follows from simple applications of L'Hospital's rule.
\end{proof}

\begin{comment}

\begin{eqnarray}
MB_M<B_n&\Rightarrow& \left(\frac{\alpha+M}{\alpha}\right)Me^{-\frac{c^2}{2\sigma_n^2}}<
\left(\frac{\alpha+n}{\alpha}\right)e^{-\frac{c^2}{2\sigma_n^2}}\nonumber\\
&\Rightarrow& M(\alpha+M)<(\alpha+n) \nonumber\\
\label{eq:BMn}
\end{eqnarray}
Assume $M(=n^b)>\alpha(=n^\omega)$, such that $M(\alpha+M)\cong M^2$ and $\alpha+n\cong n$.
Thus inequality in (\ref{eq:BMn}) holds if $M<n^{1/2}$.

\end{comment}


\begin{lemma}
\label{lemma:compare3}
$r_1(n)=\dfrac{\left(1-\frac{1}{M}\right)^n 
\left(\frac{\alpha+M}{\alpha}\right)^M}{\left(\frac{\alpha}{\alpha+n}\right)^2}\rightarrow 0$,
%if $1>b>\omega$, $b<\frac{1}{2}$.
if $\frac{1}{2}>b>\omega$.
\end{lemma}
\begin{proof}
The proof follows from simple applications of L'Hospital's rule.
\end{proof}

\begin{comment}

\begin{eqnarray}
\log(r_1(n))&=&n\log\left(1-\frac{1}{M}\right)-2\log(\frac{\alpha}{\alpha+n})-M\log(\frac{\alpha}{\alpha+M}) \nonumber\\
&=&n\log\left(1-\frac{1}{M}\right)\left[1-\frac{2\log(\frac{\alpha}{\alpha+n})}{n\log(1-\frac{1}{M})}-
\frac{M\log(\frac{\alpha}{\alpha+M})}{n\log(1-\frac{1}{M})}\right]  \nonumber\\
\label{eq:ratio1}
\end{eqnarray}


Write $\frac{\log(\frac{\alpha}{\alpha+n})}{n\log(1-\frac{1}{M})}=\dfrac{-\frac{1}{n}}{\frac{\log(1-\frac{1}{n^b})}{\log(1+n^{1-\omega})}}$.
Simple application of L'Hospital's rule shows that this ratio goes to 0 if $\omega, b <1$. Similarly we can show if
$\frac{1}{2}>b>\omega$ then $\frac{M\log(\frac{\alpha}{\alpha+M})}{n\log(1-\frac{1}{M})}\rightarrow 0$ and $n\log(1-\frac{1}{M})\rightarrow -\infty$.
Thus $\log(r_1(n)\rightarrow -\infty$, as $n\rightarrow \infty$.


Hence $r_1(n)\rightarrow 0$.\\


Since $\epsilon_M^*<\epsilon_n^*$, choosing $\frac{\epsilon_n}{1-\epsilon_n}$ such that $\epsilon_n^*\rightarrow 0$ ensures 
$\epsilon_M^*\rightarrow 0$.  we choose $\frac{\epsilon_n}{1-\epsilon_n}e^{\frac{(2a+c)^2}{2\sigma_n^2}}
\left(\frac{\alpha+M}{\alpha}\right)^M\frac{1}{B_0^M}=\frac{1}{n^{t}}$, $t>0$.\\

\begin{lemma}
\label{lemma:compare4}
If $c<b$ then $\frac{\frac{1}{M}}{\epsilon_n^*}\rightarrow 0$.
\end{lemma}


Under specified choice of $\frac{\epsilon_n}{1-\epsilon_n}$ it is easy to note that 
\begin{equation}
\frac{\frac{1}{M}}{\epsilon_n^*}=\frac{n^{t}}{n^b} \label{eq:lemma15}
\end{equation}

R.H.S of (\ref{eq:lemma15}) goes to zero if $t<b$.\\

\end{comment}

Hence, combining the results of Lemma \ref{lemma:compare1} to Lemma \ref{lemma:compare3} we conclude that 
$MISE(SB)$ converges to $0$ at a faster rate than $MISE(EW)$, provided that we choose $M$ and $\alpha$
as required by Lemmas \ref{lemma:compare1}--\ref{lemma:compare3}.
%$\frac{MISE(SB)}{MISE(EW)}\rightarrow 0$, if the conditions of 
%these lemmas hold. To get a picture the degree of difference of the two $MISE$'s we show some pictures the curve of $MISE$ against different
%choice of $n$. 

\section{Comparison with the optimal frequentist $MISE$ rate}
\label{sec:frequentist_rate}


Under suitable regularity conditions, the optimal $MISE$ rate of convergence of a kernel density
estimator is $n^{-2/5}$.
\ctn{Ghosal07} consider densities of the form
\begin{equation}
f_F(x)=\int\phi\left(\frac{x-\theta}{\sigma}\right)dF(\theta),
\label{eq:ghosal}
\end{equation}
where $F\sim D(\alpha G_0)$. Thus, in contrast to our approach where we considered predictive densities integrating out
the random measure $F$, \ctn{Ghosal07} deal with densities of the form (\ref{eq:ghosal}) 
whose randomness is induced by $F$.  
The remaining prior structure is very similar to ours.
Assuming that $f_0$ is the true density generating the data, \ctn{Ghosal07} consider convergence (to zero) under the true
distribution of the data, of posterior probabilities 
of the form $P\left(F:d_h(f_F,f_0)>C\epsilon_{0,n}\mid\bY_n\right)$, where $\epsilon_{0,n}$ is the rate of convergence
that \ctn{Ghosal07} are interested in,
$C$ is some constant and $d_h$
is some pseudo-metric; in particular, \ctn{Ghosal07} consider the Hellinger distance between two densities. 
Under certain assumptions the best rate of convergence turns to be $n^{-2/5}(\log n)^{4/5}$, 
which is slower than the frequentist $MISE$ rate. 

Here we show that in our approach, by choosing $\alpha$, $\epsilon_n$ 
and $\sigma_n$ appropriately, $MISE(SB)$ can achieve a smaller rate than $n^{-2/5}$. Moreover,
with our approach, 
$MISE(EW)$ can achieve the optimal frequentist rate $n^{-2/5}$.\\

Let $\alpha=n^\omega$, $0<\omega<1$. We set $\sigma_n^2=\frac{1}{n^t}$, $t>0$ and $\epsilon_n$ is chosen so that $\epsilon_n^*=\frac{1}{n^r}$, 
$r>0$. Then the order of $MISE(EW)$ becomes
\begin{eqnarray}
\frac{1}{\left(1+n^{1-\omega}\right)^2}+\left(\frac{\alpha+n}{\alpha}e^{-\frac{c^2n^t}{4}}\right)+\frac{1}{n^r}+\frac{1}{n^t}. 
\label{eq:mise_ew_opt1}
\end{eqnarray}
If we choose $r<\frac{2}{5}$, $t< \frac{2}{5}$ and $\omega< \frac{4}{5}$, then (\ref{eq:mise_ew_opt1}) will be less than $n^{-2/5}$. 
Moreover, under the same conditions $MISE(SB)$ has a smaller rate than $MISE(EW)$. 
The form of our true distribution satisfies the assumption of \ctn{Ghosal07} which requires
it to tend to zero smoothly at the boundary points of its support; it also satisfies those required for
frequentist density estimation. Hence, for our form of the true distribution, the convergence rates 
of the different methods are comparable--we obtain the following ordering:
$MISE(SB)\prec MISE(EW)\prec FMISE\prec BR_{GVV}$, where $FMISE$ denotes the
optimal frequentist $MISE$ rate and $BR_{GVV}$ denotes the best rate of convergence of \ctn{Ghosal07}.
%So
%we can provide a much compact bound for EW model. We have already argued that under certain conditions rate of convergence of SB model 
%is less than that of EW. So we have provided a more compact bound for SB model also.\\

We now show that for $\sigma_n=n^{-1/5}$ (which can be thought of as analogous to the optimum
bandwidth in the frequentist density estimation paradigm) $MISE(EW)$ can achieve the 
rate $n^{-2/5}$ when minimized with respect to
$\alpha$ over $0\leq\alpha<\infty$, that is, without assuming any particular form of $\alpha$.
Taking $\sigma_n^2=n^{-t}$, the order of $MISE(EW)$ is minimized for $\alpha=n\left(\dfrac{1}{1-\frac{e^{-\frac{c^2n^t}{12}}}{2^{1/3}}}-1\right)$. 
The order of $MISE(EW)$ in that case becomes 
\begin{eqnarray}
\left(\frac{1}{2^{1/3}}e^{-\frac{c^2n^t}{12}}\right)^2+2^{1/3}e^{c^2}+\frac{1}{n^r}+\frac{1}{n^t}. 
\label{eq:mise_ew_opt2}
\end{eqnarray}
Hence, if $\sigma_n^2=\frac{1}{n^{2/5}}$, then the order of $MISE(EW)$ is also 
$\frac{1}{n^{2/5}}$, if $r>t$. 

However, note that the optimum order of $MISE(EW)$ given by (\ref{eq:mise_ew_opt2}) is 
attained when $\alpha$ is a decreasing function of $n$. This is not the same condition under which we have 
proved better performance of the SB model over
the EW model. So it is of interest to study whether under this new condition also the SB model outperforms the EW model. 
Using L'Hospital's rule we can show, putting $\alpha=n\left(\dfrac{1}{1-\frac{e^{-\frac{c^2n^t}{12}}}{2^{1/3}}}-1\right)$ 
in Lemmas \ref{lemma:compare1}--\ref{lemma:compare3},
%(\ref{eq:epsilon}), (\ref{eq:BMn}) and (\ref{eq:ratio1}), 
that the corresponding ratios still converge to 0 as $n\rightarrow \infty$. Thus the SB model can achieve even smaller
optimal posterior $MISE$ rate compared to the other methods.








==> largep_smalln.tex <==


 
\section{{\bf The ``large $p$, small $n$" problem}}
\label{sec:large_p_small_n}

So far we have discussed the asymptotic performance of SB and EW models in terms of $MISE$ for univariate data. 
We now investigate the $MISE$-based convergence properties when the sample size $n$ is much smaller than $p$, the dimension of each
data point. 
In rough terms, the information contained in the data is much less compared to the number of parameters to be estimated, which
makes inference extremely challenging. 
This problem is the well-known ``large $p$, small $n$" problem.
We assume that as $n\rightarrow\infty$, $p\rightarrow\infty$ such that $p/n\rightarrow\infty$. In fact,
the data dimension should more appropriately be denoted by $p_n$, but for the sake of convenience we suppress
the suffix.
%We are now going to check the rate of convergence for EW and SB model in this problem also.


\subsection{{\bf EW model}}
\label{large_p_ew}

The EW model for $p$ variate data is defined as follows.  
\begin{equation}
Y_i\sim N_p\left(\theta_i, \Sigma\right)\ \ \mbox{independently}, \label{eq:model_ew_large}
\end{equation}
where $Y_i=(Y_{i1}, \ldots, Y_{ip})'$, $\theta_i=(\theta_{i1},\ldots,\theta_{ip})'$, $i=1, \ldots, n$ and 
%$Y_{ij}$ is independent of $Y_{il}$, $j\neq l$, 
$\Sigma=\sigma^2 I_{p\times p}$, where $I_{p\times p}$ is the $p\times p$ identity matrix.
\begin{eqnarray}
\theta_i\stackrel{iid}{\sim} F, i=1,\ldots, n; F\sim D\left(\alpha_n G_0\right), \label{eq:large_prior}
\end{eqnarray}
where $G_0$ is some fixed probability measure.
%under $G_0$, $\theta_{i}\stackrel{ind}{\sim}N_{p}\left(\mu_0, \Sigma_0\right)$, 
%where $\Sigma_0=\sigma_0^2 I_{p\times p}$;
%$\mu_0$ and $\sigma_0$ are assumed to be known. 
The prior on $\sigma$ remains the same as before. 
%Assuming that the density is supported on $[b_1, b_2]^p$, 
The density estimator at the point $y=\{y_1, \ldots, y_p\}$ is given by:

\begin{equation}
\hat f_{EW}(y\mid \Theta_n,\sigma)=\frac{\alpha}{\alpha+n}A_n
+\frac{1}{\alpha+n}\sum_{i=1}^{n} \prod_{l=1}^{p}\frac{\varphi(\theta_{il},\sigma+\hat k_n)}{(\sigma+\hat k_n)}
\phi\left(\frac{y_l-\theta_{il}}{\sigma+\hat k_n}\right).  \label{eq:large_ew_model}
\end{equation}

%Let $\bS_n=\{\bY_n:\abs {Y_{ij}}<a;i=1,\ldots,n,j=1,\ldots,p\}$.
The form of the $MISE$ and the approach to bound the $MISE$ will be same as in Section 6.1 of MB. %\ref{sec:EW_post}.
So, we proceed directly to obtain the bounds of the different parts of the $MISE$. 
The necessary lemmas are simple
%lemmas, Lemmas \ref{lemma:large_ew1} and \ref{lemma:large_ew2}, which can be thought of as 
generalizations of Lemmas \ref{lemma:epsilon_ew} and \ref{lemma:b_n_ew} 
associated with Section 6.1 of MB. %\ref{sec:EW_post}, 
%are formally stated and proved in Section \ref{subsec:proofs_largep_smalln}.
%
%
Hence, %from Lemmas S-6.1 and S-6.2 %provided in Section S-6 of the supplement
%\ref{lemma:large_ew1} and \ref{lemma:large_ew2}, 
%and from the same argument used for obtaining the 
the same approach used for obtaining
order of $MISE(EW)$ in Section 6.1 of MB, %\ref{sec:EW_post}, 
here we obtain the order of 
$MISE(EW)$ in the large $p$, small $n$ case as

\begin{equation}
E^n_0\left[MISE(EW)\right]=O\left(\left(\frac{\alpha_n}{\alpha_n+n}\right)^2+pB_n
+\epsilon_n^L+\sigma_n^2+E^n_0(\hat k_n-k)^2\right),
\label{eq:ew_order_large}
\end{equation}
where
$\epsilon_n^L=
\frac{\epsilon_n}{1-\epsilon_n}\exp\left(\frac{np(a+c_1)^2}{2{b^2_n}}\right)
\frac{(\alpha_n+n)^n}{\alpha^n_n H_0^{np}}$.


\subsection{{\bf SB model}}
\label{subsec:sb_order_large}

%Change in the SB model in Large p Small n context is almost the same as in EW model.
Here the density estimator is
\begin{equation}
\hat f_{SB}\left(y\mid \Theta_{M_n},\sigma\right)=\frac{1}{M_n}\sum_{i=1}^{M_n}\prod_{l=1}^{p}
\frac{\varphi(\theta_{il},\sigma+\hat k_n)}{(\sigma+\hat k_n)}
\phi\left(\frac{y_l-\theta_{il}}{\sigma+\hat k_n}\right),  \label{eq:large_sb_model}
\end{equation}
where $\Theta_{M_n}=\left(\theta_1,\ldots,\theta_{M_n}\right)'$, $\theta_i=(\theta_{i1}, \ldots, \theta_{ip})'$, 
$\Sigma=\sigma^2 I_{p\times p}$.  
%the prior assumptions are the same as in equations (\ref{eq:model_ew_large}) and (\ref{eq:large_prior}).  
We assume that $\theta_i\stackrel{iid}{\sim}F$ and $F\sim DP(\alpha_n G_0)$, and 
$y_i\stackrel{iid}{\sim}\hat f_{SB}\left(\cdot\mid \Theta_{M_n},\sigma\right)$.


We bound the individual probabilities in the same way as in Section 6.2 of MB. %\ref{sec:sb_model}; 
%see
%Lemmas S-7.1, S-7.2, S-7.3, and S-7.4.
%Lemmas \ref{lemma:sb_lemma18}, \ref{lemma:sb_lemma19}, \ref{lemma:sb_lemma20}, and \ref{lemma:sb_lemma21}.
%
%
%
%Let $E=$\{all $\theta_l$'s in likelihood are in $[-a-c,a+c]$, rest are in $\Re^p$\}.
% 
%
%
Proceeding in the same way as in Section 6.2 of MB %\ref{sec:sb_model} 
we can show that the order of $MISE$ of SB model for the 
``large $p$, small $n$" case is
\begin{eqnarray}
E^n_0\left[MISE(SB)\mathbb I_{\bS_n}\right]=O\left(\left(1-\frac{1}{M_n}\right)^n 
\left(\frac{\alpha_n+M_n}{\alpha_n}\right)^{M_n}+M_npB_{M_n}+\epsilon_{M_n}^L+\sigma_n^2+E^n_0(\hat k_n-k)^2\right), \nonumber\\
\label{eq:sb_order_large}
\end{eqnarray}
where
$\epsilon_{M_n}^L=\frac{\epsilon_n}{1-\epsilon_n}\exp\left(\frac{np(a+c_1)^2}{2(b_n)^2}\right)
\frac{(\alpha_n+M_n)^{M_n}}{(\alpha_n)^{M_n} H_0^{M_np}}$.


Note that the two ``large $p$, small $n$" $MISE$'s given by (\ref{eq:ew_order_large}) and (\ref{eq:sb_order_large}) converge to zero 
if $\sigma_n$ and $\epsilon_n$ converge to 
zero at a much faster rate than the rate needed for $MISE$'s given by 
%(29) and (34) of MB.
(28) and (33) of MB.
%(\ref{eq:mise_order_ew}) and (\ref{eq:mise_order_sb}). 
%Note that $p\gg n$, 
This is clear because $p$ grows much faster than $n$ and so, the terms $pB_n$ and $M_npB_{M_n}$ 
involved in the $MISE$'s 
do not go to zero unless $\sigma_n$ is made to converge to zero much faster than in the usual cases. 
Also, $\epsilon_n$ must go to zero much faster than in the usual situations to ensure that $\epsilon^L_n$
and $\epsilon^L_{M_n}$ converge to zero. In other words, rather strong prior information is necessary to 
compensate for the deficiency of information in the data.

The above arguments show that even in the ``large $p$, small
$n$" problem both EW and SB model can be consistent in terms of $MISE$ by choosing the prior on $\sigma$ appropriately. 
However, it is easy to see that even in this set-up, $MISE(SB)\prec MISE(EW)$.


It is also clear that all our ``large $p$, small $n$" asymptotic results related to the SB density estimator
(\ref{eq:large_sb_model}) and the asymptotic comparisons with the corresponding EW density estimator 
(\ref{eq:large_ew_model}) remain exactly the same if the discrete weights $1/M$ are replaced with 
continous weights $\pi_i$ as in Section 9 of MB.







==> prior_predictive.tex <==

\section{Prior predictive convergence rates}
\label{sec:prior_predictive}


\subsection{Models under consideration}


\subsubsection{Assumptions on the true distribution}

Let $f_0$ denote the true distribution.
We assume that $f_0$ is continuously differentiable of all orders.
Thus, the assumptions on $f_0$ for the prior calculations are different from those
associated with the posterior calculations.

\subsubsection{EW model}
\label{sec:ew_model}


We denote $\Theta_n=\{\theta_1, \ldots, \theta_n\}$ and assume $\theta_i\stackrel{iid}{\sim}F$ and $F\sim D(\alpha_n G_0)$, where $D(\alpha_n G_0)$
denotes the Dirichlet process with central measure $G_0$ and hyperparameter $\alpha_n$. 
Then, according to the EW model, the prior predictive density at the point $y$ has the following form:
\begin{equation}
\hat f_{EW}(y\mid \Theta_n,h)=\frac{\alpha_n}{\alpha_n+n}A+\frac{1}{\alpha_n+n}
\sum_{i=1}^{n}\frac{1}{h}K\left(\frac{y-\theta_i}{h}\right),
\label{eq:ew_model_prior}
\end{equation}
where we assume the kernel $K(\cdot)$ to be symmetric around zero, 
$A=\int_{\theta}\frac{1}{h}K\left(\frac{y-\theta}{h}\right)G_0(\theta)d\theta$. 
In our work on calculating prior rates, we determine the optimum value of $h$ by minimizing the rate of convergence. 


\subsubsection{SB model}
\label{subsubsec:sb_model}

The SB model assumes that the density at the point $y$ is given by,
\begin{equation}
\hat f_{SB}(y\mid \Theta_{M_n},h) = \frac{1}{M_n} \sum_{l=1}^{M_n} \frac{1}{h}K\left(\frac{y-\theta_l}{h}\right),
\label{eq:sb_model_prior}
\end{equation}
where for each $l$, $\theta_l\sim F$; $F\sim D(\alpha_n G_0)$, $\Theta_{M_n}=\{\theta_1, \ldots, \theta_{M_n}\}$; $M_n$ being the maximum number of distinct
components the mixture model can have.
In both EW and SB models, we confine attention to the case where $K(\cdot)$ is chosen to be the $N(0, 1)$ density.



\subsection{Measure of divergence}
\label{eq:measure_diverge}

To study the rates of convergence we need to define a measure of divergence. In our study we use the 
$MISE$ as the measure of divergence, defined as,
\begin{eqnarray}
\label{eq:MISE}
MISE &=& \int_{y}E(\hat f(y\mid \Theta)-f(y))^2dy \\
&=& \int_{y}\int_{\Theta} \left\{\hat f(y\mid \Theta)-f(y)\right\}^2dH(\Theta)dy, \nonumber
\end{eqnarray}
where the expectation is taken over $\Theta$, the set of parameters of the model and $H(\cdot)$ is the joint distribution of 
$\Theta$ obtained by integrating out the unknown random measure $F$. Since $F$ is a Dirichlet process in our case,
$H(\cdot)$ is composed of the Polya urn distributions. As mentioned before, $h$ will be determined by minimizing $MISE$. 



We have assumed $h$ to be non-random and determine it by minimizing $MISE$ given in
(\ref{eq:MISE}). We begin with the assumption that $G_0(\cdot) = f(\cdot)$. This assumption
is more pedagogical than practical but we will show subsequently that the prior convergence rate 
remains unchanged under less restrictive assumptions on $G_0$.
Of course, it is most appropriate to study the posterior convergence rate since the information contained in
the data ensures that the resultant calculations are valid under far greater generality; in fact, restrictive
assumptions on $G_0$ are not necessary at all. %Although we have focused on posterior calculations in this work, 
However, since in the Bayesian paradigm it is often recommended that the prior parameters be chosen before 
observing the data, it perhaps makes sense to choose values of the prior parameters which keep the prior 
$MISE$ rates 
at the desired level. 


Since EW is a special case of SB, we begin by calculating the $MISE$ for the SB model; that for EW will follow
quite simply then. 

\subsubsection{Calculations}
\label{eq:cal_mise}

\begin{eqnarray}
MISE &=& \int_yE(\hat f_{SB}(y\mid \Theta_{M_n},h)-f(y))^2dy \nonumber\\
&=& \int_{y}\int_{\Theta_{M_n}} \left\{\frac{1}{M_n}\sum_{l=1}^{M_n} \frac{1}{h}K\left(\frac{y-\theta_l}{h}\right)
-f(y) \right\}^2dH\left(\Theta_{M_n}\right) dy \nonumber\\
&=& \int_y Var\left(\hat f_{SB}\left(y\mid \Theta_{M_n},h\right)\right)dy + \int_{y} \left\{bias_h(y)\right\}^2dy, \nonumber\\
\end{eqnarray}
where $bias_h(y) = \left\{E\left(\hat f_{SB}\left(y\mid
\Theta_{M_n},h\right)\right)-f(y)\right\}$ and
$H\left(\Theta_{M_n}\right)$ is the joint distribution of $\Theta_{M_n}$.
We write,
\begin{equation}
bias_h(y) = \int h^{-1} K\left(\frac{y-x}{h}\right) G_0(x)dx - f(y) \nonumber
\end{equation}
Calculations similar to those in \ctn{Silverman86} yield

\begin{comment}
M_naking the change of variable $t = (y-x)/h$ and using $\int K(x) dx = 1$, we can write,
\begin{eqnarray}
bias_h(y) &=& \int K(t)f(y-ht)dt - f(y) \nonumber\\
&=& \int K(t) \left\{f(y)-htf^{'}(y)+\frac{1}{2}h^2t^2f^{''}(y)-\cdots\right\}dt - f(y), \nonumber\\
\label{eq:expand_bias}
\end{eqnarray} 
using Taylor series expansion of $f(y-ht)$.
By symmetry of $K(\cdot)$ around 0, $\int tK(t)dt = 0$ and hence 
\begin{eqnarray}
bias_h(y)
= \frac{1}{2}h^2k_2f^{''}(y) + O(h^3), \nonumber\\
\end{eqnarray}
where $k_2 = \int t^2K(t)dt$.
So, $O(bias_h(y)) = O(h^{2})$. %Ignoring the term of order $O(h^3)$, we have
It is easy to see that 
\end{comment}
\begin{equation}
\int \left(bias_h(y)\right)^2dy = O(h^4) 
\label{eq:bias}
\end{equation}

Now, the variance term can be expressed as
\begin{eqnarray}
&&Var(\hat f_{SB}(y\mid \Theta_{M_n},h))  \nonumber\\ 
&=& \frac{1}{M_n^2h^2}\sum_{j=1}^{M_n} Var\left(K\left(\frac{y-\theta_j}{h}\right)\right)+ \nonumber\\
&& \frac{1}{M_n^2h^2}\sum_{j=1}^{M_n}\sum_{l=1,l\neq j}^{M_n} Cov\left(K\left(\frac{y-\theta_j}{h}\right), K\left(\frac{y-\theta_l}{h}\right)\right) 
\nonumber
\end{eqnarray}
Now, assuming that $h$ is small and $M_n$ is large, and expanding $f(y-th)$ as a Taylor series we obtain
\begin{comment}
\begin{eqnarray}
&&\frac{1}{M_nh^2}Var(K((y-\theta_j)/h)) \nonumber\\
&=& \frac{1}{M_nh}\int K^2(t)f(y-ht)dt + O(M_n^{-1}) \nonumber\\
&\approx& \frac{1}{M_nh}
\int K^2(t)\left\{f(y)-htf^{'}(y)+\frac{1}{2}h^2t^2f^{''}(y)-\cdots\right\}dt \nonumber\\
&\approx& \frac{1}{M_nh}f(y) \int K^2(t)dt 
\label{eq:assump}
\end{eqnarray}
Since $f(y)$ is a density function $\int f(y)dy = 1$. Thus,
\begin{equation}
\int \frac{1}{M_n^2h^2}\sum_{j=1}^{M_n} Var\left(K\left(\frac{y-\theta_j}{h}\right)\right)dy\approx \frac{1}{M_nh}\int K^2(t)dt
\label{eq:var}
\end{equation}
\end{comment}
\begin{equation}
\int \frac{1}{M_n^2h^2}\sum_{j=1}^{M_n} Var\left(K\left(\frac{y-\theta_j}{h}\right)\right)dy=O\left(\frac{1}{M_nh}\right)
\label{eq:var}
\end{equation}


For the covariance term,
\begin{eqnarray}
&&\frac{1}{M_n^2h^2}\sum_{j}\sum_{l\neq j} Cov\left(K\left(\frac{y-\theta_j}{h}\right), K\left(\frac{y-\theta_l}{h}\right)\right)\nonumber\\
&=&\frac{M_n(M_n-1)}{M_n^2h^2} Cov\left(K\left(\frac{y-\theta_1}{h}\right), K\left(\frac{y-\theta_2}{h}\right)\right) \nonumber\\
&=& \left(1-\frac{1}{M_n}\right)\frac{1}{h^2} Cov\left(K\left(\frac{y-\theta_1}{h}\right), K\left(\frac{y-\theta_2}{h}\right)\right) \nonumber\\
&\leq& \frac{1}{h^2} Cov\left(K\left(\frac{y-\theta_1}{h}\right), K\left(\frac{y-\theta_2}{h}\right)\right).  \nonumber\\
\label{eq:main_cov} 
\end{eqnarray} 
%taking $M_n$ to be large enough so that we can ignore terms of the order $\frac{1}{M_n}$ or terms higher than this.


Simple calculations, using Taylor's series expansion yields
\begin{equation}
\int_{y} \frac{1}{h^2}Cov\left(K\left(\frac{y-\theta_j}{h}\right), K\left(\frac{y-\theta_l}{h}\right)\right)dy 
=O\left(\frac{1}{\alpha_n+1}\right).
\label{eq:var_f}
\end{equation}


From (\ref{eq:bias}), (\ref{eq:var}) and (\ref{eq:var_f}) we conclude that

\begin{equation}
MISE(SB)=O\left(\frac{1}{M_nh}+\frac{1}{\alpha_n+1}+h^4\right).
\label{eq:prior_mise_sb}
\end{equation}
We will assume $M_n$ and $\alpha_n$ to be functions of $n$ and will determine $h$ as a function of $n$ 
by minimizing the above form of $MISE$. 
The resultant form of $MISE$ will be compared with that corresponding to the EW model.


\subsection{Determination of $h$}
\label{eq:determin_h}

Minimizing (\ref{eq:prior_mise_sb}) with respect to $h$ yields $h_{opt}=O\left(M_n^{-\frac{1}{5}}\right)$.
Plugging $h_{opt}$ in (\ref{eq:prior_mise_sb}) gives the optimal order of $MISE(SB)$:
\begin{equation}
MISE(SB)_{opt}=O\left(\frac{1}{\alpha_n+1}+M_n^{-\frac{4}{5}}\right)
\label{eq:prior_mise_sb_opt}
\end{equation}
Choosing $\alpha_n=O\left(M_n^{\lambda}\right)$ we get $MISE(SB)_{opt}=O\left(M_n^{-\lambda}\right)$
if $\lambda<\frac{4}{5}$ and $O\left(M_n^{-\frac{4}{5}}\right)$ if $\lambda\geq\frac{4}{5}$.

\subsection{Extension to a more general situation}
\label{subsec:prior_general}

In the prior-based MISE calculated so far we have assumed that $G_0(\cdot)=f(\cdot)$.
Let us now assume a more general situation where 
$G_0(\theta) = \frac{1}{M_n}g(\theta)+\left(1-\frac{1}{M_n}\right)f(\theta)$, 
where $g(\cdot)$ is a density different from the true density $f(\cdot)$.  
It can be easily shown that here also the order of $MISE(SB)$ and $MISE(SB)_{opt}$ 
remain of the form as (\ref{eq:prior_mise_sb}) and (\ref{eq:prior_mise_sb_opt}) respectively.





\subsection{Prior convergence rates of the EW model}
\label{subsec:prior_predictive_ew}
The form of the predictive distribution of EW is
\begin{equation}
\hat f_{EW}(y\mid \Theta_n,h)=\frac{\alpha_n}{\alpha_n+n}A+\frac{1}{\alpha_n+n}\sum_{i=1}^{n}\frac{1}{h}K\left(\frac{y-\theta_i}{h}\right).  \nonumber
\end{equation}

Note that the conditional distribution of $\theta_i$ given $\Theta_{-in}\left(=\Theta_n\setminus\theta_i\right)$ is given by
$\frac{\alpha_n}{\alpha_n+n}G_0(\theta_i)+\frac{1}{\alpha_n+n}\sum_{l=1, l\neq i}^{n}\delta_{\theta_l}(\theta_i)$. 
Suppose $\alpha_n=O\left(n^{\omega}\right)$. If we choose $\omega>1$, then $\frac{\alpha_n}{\alpha_n+n}\rightarrow 1$. This will imply that
the conditional distribution $\theta_i$ given $\Theta_{-in}$ is close to $G_0(\theta_i)$ for large $n$. This fact will defeat the basic goal 
of using nonparametric prior. Thus we will set $\omega< 1$ and choose $\alpha_n$
such that $\frac{n}{\alpha_n+n}\rightarrow 1$. Thus for large $n$ the model will look like
$\frac{1}{\alpha_n+n}\sum_{i=1}^{n}\frac{1}{h}K\left(\frac{y-\theta_{i}}{h}\right)$, the form similar to our form in (\ref{eq:sb_model_prior}).
Calculations similar to those associated with the $MISE$ of the SB model show that for the EW model the $MISE$ is
given by

\begin{comment}
\begin{eqnarray}
&&MISE(EW) \nonumber\\
&=&\frac{1}{(\alpha_n+n)h}\int K^2(t)dt+
\left(\frac{1}{\alpha_n+1}\int K^2(t)dt-\frac{1}{\alpha_n+1}\int_{y} f^2(y)dy\right)+ \nonumber\\
&&\frac{1}{4}h^4k_{2}^2 \int (f^{''}(y))^2dy,
\label{eq:mise_ew}
\end{eqnarray}
assuming $\frac{n}{\alpha_n+n}\approx 1$.\\
\end{comment}

\begin{equation}
MISE(EW) = O\left(\frac{1}{(\alpha_n+n)h}+\frac{1}{\alpha_n+1}+h^4\right)
\label{eq:mise_ew}
\end{equation}

Minimizing this form of $MISE$ yields $h_{opt}$ which is of the order $\frac{1}{(\alpha_n+n)^{1/5}}$. Plugging $h_{opt}$ in $MISE(EW)$
gives $MISE(EW)_{opt}=O\left(\frac{1}{(\alpha_n+n)^{4/5}}+\frac{1}{\alpha_n+1}\right)$.


Note that the order of $MISE(EW)$ is less than that of $MISE(SB)$ unless $M_n>n$. This is to be expected 
since so far our calculations are with respect to the prior only, not involving the data; hence, more the
number of components in the mixture model faster the rate of convergence. 

\section{Comparison between prior and posterior convergence rates}
\label{sec:comparison_prior}


To provide a feel for the prior and the posterior rates associated with the two competing models of 
EW and SB, we present plots of the orders of $MISE(EW)$ and $MISE(SB)$ for both prior and posterior
predictive cases, for appropriate values of the parameters involved in the rates of convergence.

We assume the following forms:
$M_n=n^{b}$, $\alpha_n=n^{\omega}$, %$0<\omega<1$, $0<b<1$ and $\omega<b<\frac{1}{2}$. 
%Further, we set 
$\sigma_n^2=\frac{c^2}{4e^{n^t}}$, 
$\epsilon_n^*=\frac{1}{n^r}$, where $r=3$, and $t>0$ (the $MISE$'s will be compared for different
values of $t$). By equating $\epsilon_n^*=\frac{1}{n^r}$, we can calculate the value of $\frac{\epsilon_n}{1-\epsilon_n}$
which is used get closed form expression for $\epsilon_{M_n}^{*}$.
In the above forms we assume that %$\omega=3.5$, 
$b=0.2$, $\mu_0=2.0$, and $\sigma_0=1.0$. 
For different values of $t$ and $\omega$, figures \ref{fig:compare_ew1} and \ref{fig:compare_ew2}
present and compare the prior based rates of $MISE(EW)$ and $MISE(EW)$ for different values
of $t$ and $r$. On the other hand, figures \ref{fig:compare_sb1} and \ref{fig:compare_sb2}
compare the $MISE$ rates of EW and SB based on the posterior. 

As already discussed in Section \ref{subsec:prior_predictive_ew}, figures \ref{fig:compare_ew1} 
and \ref{fig:compare_ew2} show that the prior EW rates are faster than the prior SB rates, 
which is expected, since, in this illustration, $M_n<n$. On the other hand, the figures
\ref{fig:compare_sb1} and \ref{fig:compare_sb2} show that the posterior SB rates are far superior
to the posterior EW rates. 
\begin{figure}
\begin{center}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_05_1_new_prior}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_05_2_new_prior}
\caption{Prior predictive case with $\omega=0.05$. The black curve corresponds to the 
prior predictive $MISE$ of the EW model and the red curve 
corresponds to that of the SB model. The left and the right panel correspond to $t=2$ and $t=5$,
respectively.}
\label{fig:compare_ew1}
\end{center}
%\end{figure}
%\begin{figure}
\begin{center}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_1_1_new_prior}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_1_2_new_prior}
\caption{Prior predictive case with $\omega=0.1$. The black curve corresponds to the 
prior predictive $MISE$ of the EW model and the red curve 
corresponds to that of the SB model. The left and the right panel correspond to $t=2$ and $t=5$,
respectively.}
\label{fig:compare_ew2}
\end{center}
\end{figure}
\begin{figure}
\begin{center}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_05_1_new_post}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_05_2_new_post}
\caption{Posterior predictive case with $\omega=0.05$. The black curve corresponds to the 
prior predictive $MISE$ of the EW model and the red curve 
corresponds to that of the SB model. The left and the right panel correspond to $t=2$ and $t=5$,
respectively.}
\label{fig:compare_sb1}
\end{center}
%\end{figure}
%\begin{figure}
\begin{center}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_1_1_new_post}
\includegraphics[width = 6cm, height = 7cm]{plots/a0_1_2_new_post}
\caption{Posterior predictive case with $\omega=0.1$. The black curve corresponds to the 
prior predictive $MISE$ of the EW model and the red curve 
corresponds to that of the SB model. The left and the right panel correspond to $t=2$ and $t=5$,
respectively.}
\label{fig:compare_sb2}
\end{center}
\end{figure}


